A Sequential Composition Framework for Coordinating Multi-Robot Behaviors

A number of coordinated behaviors have been proposed for achieving specific tasks for multi-robot systems. However, since most applications require more than one such behavior, one needs to be able to compose together sequences of behaviors while respecting local information flow constraints. Specifically, when the inter-agent communication depends on inter-robot distances, these constraints translate into particular configurations that must be reached in finite time in order for the system to be able to transition between the behaviors. To this end, we develop a distributed framework based on finite-time convergence control barrier functions that enables a team of robots to adjust its configuration in order to meet the communication requirements for the different tasks. In order to demonstrate the significance of the proposed framework, we implemented a full-scale scenario where a team of eight planar robots explore an urban environment in order to localize and rescue a subject.

==> sections/controllers.tex <==
\section{Behaviors Dynamic} \label{sec:appendixB}
\paragraph{Rendezvous}
\begin{equation}
	u_i = \sum_{j \in \mathcal{N}_i} x_j - x_i
\end{equation}

\paragraph{Scatter}
\begin{equation}
	u_i = \sum_{j \in \mathcal{N}_i} x_i - x_j
\end{equation}


\paragraph{Formation control}
\begin{equation}
	u_i = \sum_{j \in \mathcal{N}_i} (\|x_i-x_j\|^2-\theta_{ij}^2)(x_j - x_i)
\end{equation}

where $\theta_{ij}$ must be feasible.

\paragraph{Leader-follower}
\begin{align}
	u_f &= \sum_{j \in \mathcal{N}_i} (\|x_i-x_j\|^2-\theta_{ij}^2)(x_j - x_i) \\
	u_l &= \sum_{j \in \mathcal{N}_i} \left( (\|x_i-x_j\|^2-\theta_{ij}^2)(x_i - x_i) \right) + \gamma_g(x_g-x_i) 
\end{align}

\paragraph{Leader formation}
\begin{align}
	u_f &= \sum_{j \in \mathcal{N}_i} (\|x_i-x_j\|^2-\theta_{ij}^2)(x_j - x_i) \\
	u_l &= \sum_{j \in \mathcal{N}_i} \left( (\|x_i-x_j\|^2-\theta_{ij}^2)(x_i - x_i) \right) + \gamma_g(x_g-x_i) 
\end{align}
where $\theta_{ij}$ must be feasible.

\paragraph{Cyclic pursuit}
\begin{equation}
	u_i = \sum_{j \in \mathcal{N}_i} R(\theta)\,(x_j - x_i) 
\end{equation}
where $\mathcal{G}$ must be $C_N$ (cycle graph).

\paragraph{Lattice}
\begin{equation}
u_i = \sum_{j \in \mathcal{N}_i} (\|x_i-x_j\|^2-\theta^2)(x_j - x_i)
\end{equation}
where $\theta \simeq 0.8$ max sensing radius. 

\paragraph{Coverage}
\begin{equation}
u_i = c_i - x_i
\end{equation}
where $c_i$ centroid of Voronoi tessellation.

\paragraph{Swarming}
\begin{equation}
u_i = \sum_{j \in \mathcal{N}_i} \dots (x_j - x_i)
\end{equation}

